mBART: Multidimensional Monotone BART

For the discovery of regression relationships between Y and a large set of p potential predictors x 1 , . . . , x p , the flexible nonparametric nature of BART (Bayesian Additive Regression Trees) allows for a much richer set of possibilities than restrictive parametric approaches. However, subject matter considerations sometimes warrant a minimal assumption of monotonicity in at least some of the predictors. For such contexts, we introduce mBART, a constrained version of BART that can flexibly incorporate monotonicity in any predesignated subset of predictors using a multivariate basis of monotone trees, while avoiding the further confines of a full parametric form. For such monotone relationships, mBART provides (i) function estimates that are smoother and more interpretable, (ii) better out-of-sample predictive performance, and (iii) less post-data uncertainty. While many key aspects of the unconstrained BART model carry over directly to mBART, the introduction of monotonicity constraints necessitates a fundamental rethinking of how the model is implemented. In particular, the original BART Markov Chain Monte Carlo algorithm relied on a conditional conjugacy that is no longer available in a monotonically constrained space. Various simulated and real examples demonstrate the wide ranging potential of mBART.

==> references.tex <==


%\begin{center}
%{\bf References}
%\end{center}

\section*{References}
\renewcommand{\baselinestretch}{1.00}

\begin{description} \small

\item \textsc{Azzalini, A}. (1985). A class of distributions which includes the normal ones. {\sl Scand. J. Statist.} {\bf 12} 171-178.

\item \textsc{Barlow, R.E.}, \textsc{Bartholomew, D.}, \textsc{Bremner, J.M.} and \textsc{Brunk, H.D.} (1972). {\sl Statistical Inference Under Order Restrictions: Theory and Application of Isotonic Regression.} New York: Wiley.

\item \textsc{Bleich, J.}, \textsc{Kapelner, A.}, \textsc{George, E.I.} and \textsc{Jensen, S.T.} (2014). Variable selection for BART: An application to gene regulation. {\sl Ann. Appl. Stat.} {\bf 8} 1750-1781.

\item \textsc{Cai, B.} and \textsc{Dunson, D. B.} (2007). Bayesian multivariate isotonic regression splines: applications to carcinogenicity studies. {\sl J. Amer. Statist. Assoc.} {\bf 102} 1158-1171. 

\item \textsc{Chen, Y.} and \textsc{Samworth, R.J.} (2016). 
Generalized additive and index models with shape constraints. {\sl J. R. Statist. Soc. B} {\bf 78} 729--754.

\item \textsc{Chernozhukov, V.}, \textsc{Fernandez-Val, I}. and \textsc{Galichon, A.} (2009).  
Improving point and interval estimators of monotone functions by rearrangement. {\sl Biometrika} 96, 3, pp. 559--575.

\item \textsc{Chipman, H.}, \textsc{George, E.I.} and \textsc{McCulloch, R.E.} (1998). Bayesian CART model search (with discussion and a rejoinder by the authors). {\sl J. Amer. Statist. Assoc.} {\bf 93} 935-960.

\item \textsc{Chipman, H.}, \textsc{George, E.I.} and \textsc{McCulloch, R.E.} (2010). BART: Bayesian additive regression trees. {\sl Ann. Appl. Stat.} {\bf 4} 266-298.

\item \textsc{Chipman, H.}, \textsc{George, E.I.} and \textsc{McCulloch, R.E.} (2013). Bayesian Regression Structure Discovery.
{\sl In Bayesian Theory and Applications}, (Eds, P. Damien, P. Dellaportas, N. Polson, D. Stephens), Oxford University Press, USA.

\item \textsc{Holmes, C.C.} and \textsc{Heard, N.A.} (2003). Generalized monotonic regression using random change points. {\sl Statist. Med.} {\bf 22} 623-638.

\item \textsc{Kapelner, A.} and \textsc{Bleich, J.} (2016). bartMachine: Machine learning with Bayesian additive regression trees. {\sl J. Stat. Softw.} {\bf 70} 1-40.

\item \textsc{Kong, M.} and \textsc{Eubank, R.L.} (2006). Monotone smoothing with application to dose-response curve. {\sl Commun. Statist. B-Simul.} {\bf 35} 991-1004.

\item \textsc{Lavine, M.} and \textsc{Mockus, A.} (1995). A nonparametric Bayes method for isotonic regression.
{\sl J. Stat. Plan. Inference}. {\bf 46}, 235-248.

\item \textsc{Lenk, P.J.} and \textsc{Choi, T.}  (2017).   Bayesian analysis of shape-restricted functions using Gaussian process priors.  {\sl Statistica Sinica} {\bf 27} 43-69.

\item \textsc{Lin, L.} and \textsc{Dunson, D.B.} (2014). Bayesian monotone regression using Gaussian process projection. {\sl Biometrika} {\bf 101} 303-317.

\item \textsc{Lin, L.}, \textsc{St.~Thomas, B.}, \textsc{Piegorsch, W.W.}, \textsc{Scott, J.} and \textsc{Carvalho, C.} (2019). A Projection Approach For Multiple Monotone Regression.  ArXiv:1911.07553.

\item \textsc{Linero, A.R.} and \textsc{Yang, Y.} (2018). Bayesian Regression Tree Ensembles that Adapt to Smoothness and Sparsity.  {\sl J. R. Statist. Soc. B} \,{\bf 80} 1087--1110.

\item \textsc{Mammen, E.} (1991). Estimating a smooth monotone regression function. {\sl Ann. Statist.} {\bf 19} 724-740.

\item \textsc{Meyer, M. C.}, \textsc{Hackstadt, A. J.} and \textsc{Hoeting, J. A.} (2011). Bayesian estimation and inference for generalised partial linear models using shape-restricted splines. {\sl J. Nonparam. Statist.} {\bf 23} 867--884.

\item \textsc{Neelon, B.} and \textsc{Dunson, D.B.} (2004). Bayesian isotonic regression and trend analysis. {\sl Biometrics} {\bf 60} 177-191. 
 
\item \textsc{Ramsay, J.O.} (1998). Estimating smooth monotone functions. {\sl J. R. Statist. Soc. B} {\bf 60} 365-375.

\item \textsc{Rockova, V.} and \textsc{Saha, E.}  (2019). On Theory for BART. {\sl Proceedings of the $22^{nd}$ International Conference on Artificial Intelligence and Statistics} {\bf 89}  2839--2848.

\item \textsc{Rockova, V.} and \textsc{van der Pas, S.} (2020). Posterior Concentration for Bayesian Regression Trees and Forests. {\sl Ann. Statist.}  48(4) 2108Ð-2131.

\item \textsc{Saarela, O.} and \textsc{Arjas, E.} (2011). A method for Bayesian monotonic multiple regression. {\sl Scand. J. Statist.} {\bf 38} 499-513.

\item \textsc{Salomond, J.} (2014).  Concentration rate and consistency of the
posterior distribution for selected priors under monotonicity constraints. {\sl Electronic Journal of Statistics}
Vol. 8  1 1380--1404.

\item \textsc{Shively, T.S.}, \textsc{Sager, T.W.} and \textsc{Walker, S.G.} (2009). A Bayesian approach to nonparametric monotone function estimation. {\sl J. R. Statist. Soc. B} {\bf 71} 159-175.

\item \textsc{Shively, T.S.}, \textsc{Walker, S.G.} and \textsc{Damien, P.} (2011). Nonparametric function estimation subject to monotonicity, convexity and other shape constraints. {\sl J. Econometrics} {\bf 161} 166--81.

\item \textsc{Wang, W.} and \textsc{Welch, W.} (2018).  Bayesian optimization using monotonicity information and its application in machine learning hyperparameter tuning.  {\sl Proceedings of the ICML 2018 AutoML Workshop}  1-8.

\item \textsc{Wang, X.} and \textsc{Berger, J.O.} (2016). Estimating Shape Constrained Functions Using Gaussian Processes. {\sl  J. Uncertainty Quantification} {\bf 4} 1--25.

\item \textsc{Westling, T.} \textsc{van der Laan, M. J.} and \textsc{Carone,M.} (2020). Correcting an estimator of a multivariate monotone function with isotonic regression. {\sl Electron. J. Statist.} 14 2 3032--3069.


\end{description}


